Stereo 3D Object Trajectory Reconstruction

We present a method to reconstruct the three-dimensional trajectory of a moving instance of a known object category using stereo video data. We track the two-dimensional shape of objects on pixel level exploiting instance-aware semantic segmentation techniques and optical flow cues. We apply Structure from Motion (SfM) techniques to object and background images to determine for each frame initial camera poses relative to object instances and background structures. We refine the initial SfM results by integrating stereo camera constraints exploiting factor graphs. We compute the object trajectory by combining object and background camera pose information. In contrast to stereo matching methods, our approach leverages temporal adjacent views for object point triangulation. As opposed to monocular trajectory reconstruction approaches, our method shows no degenerated cases. We evaluate our approach using publicly available video data of vehicles in urban scenes.

==> methods_object_motion_stereo_constraint_set_up_figure.tex <==

\begin{figure}[!t]
	\centering
	\begin{tikzpicture}[
	axisGlobal/.style={>=latex,draw=black,fill=black},
	xAxisLocal/.style={>=latex,draw=red,fill=red},
	zAxisLocal/.style={>=latex,draw=black,fill=black},
	plane/.style={draw=black,fill=blue!10},
	string/.style={draw=red, thick},
	]
	
	\draw[axisGlobal,->] (0,0) -- +(5.5,0) node[above] {$x$};
	\draw[axisGlobal,->] (0,0) -- +(0,1.5) node[above] {$z$};
	
	\draw[plane] (0.5,0.5) coordinate (startLeft) -- +(1,0) -- +(0.5,-0.5) coordinate (centerLeft) -- cycle;
	%\draw[xAxisLocal,->] (centerLeft) -- +(1,0) node[above, text=red] {$x_l$};
	\draw[zAxisLocal,->] (centerLeft) -- +(0,1) node[above, text=black] {$\vec{n}_l$};
	\path (centerLeft) ++(0,-0.3) node {$c_l$};
	
	\draw[plane] (startLeft)++(2.5,0) -- +(1,0) -- +(0.5,-0.5) coordinate (centerRight) -- cycle;
	%\draw[xAxisLocal,->] (centerRight) -- +(1,0) node[above, text=red] {$x_r$};
	\draw[zAxisLocal,->] (centerRight) -- +(0,1) node[above, text=black] {$\vec{n}_r$};
	\path (centerRight) ++(0,-0.3) node {$c_r$};
	
	\draw[<->] (centerLeft)+(0,-0.6) -- ($(0,-0.6)+(centerRight)$) node[pos=0.5, below] {$b$};	
	
	\end{tikzpicture}
	% Definition, setup, nomenklatur, bezeichnung, 
	\caption{Relation of the coordinate systems of the stereo camera system. $c_l$ and $c_r$ denote the camera centers of the left and right camera and $b$ denotes the corresponding baseline. $x$ and $z$ are the coordinate axis of the stereo camera system.}
	\label{methods:stereo_set_up}
\end{figure}

==> methods_object_motion_stereo_sorting.tex <==
Due to camera registration errors during the SfM reconstruction process not all stereo camera pairs are suitable to determine the scale ratio $r$ using equation \eqref{eq:final_ratio}. This is mainly the case for object reconstructions. Due to small object sizes and reflecting object surfaces the registration of cameras is less stable compared to background reconstructions. See Fig.~\ref{methods:registration_error_example} for example.\\
Without the loss of generality, we assume that the stereo camera system is organized according to Fig.~\ref{methods:stereo_set_up}. Both cameras are looking along the positive $z$ axis of the stereo camera system, i.e. the viewing directions $\vec{n}_{l}$ and $\vec{n}_{r}$ are parallel to the $z$ axis. The right camera center shows an offset of $b$ along the $x$ axis w.r.t. the left camera center. The up-vectors $\vec{u}_{l}$ and $\vec{u}_{r}$ of the left and the right camera are parallel to the $y$ axis. We use the following metrics to evaluate the quality of a registered stereo cameras in the object reconstruction. We define the \emph{normal projection error} $\delta_{\vec{n}}$ according equation \eqref{eq:stereo_z_projection}
\begin{equation}
\label{eq:stereo_z_projection}
\delta_{\vec{n},i} = \sqrt{\left( \vec{n}_{i,l}^{(o)} \cdot (\vec{c}_{i,l}^{(o)} - \vec{c}_{i,r}^{(o)}) \right)^{2} + \left(\vec{n}_{i,r}^{(o)} \cdot (\vec{c}_{i,r}^{(o)} - \vec{c}_{i,l}^{(o)})\right)^{2}}
\end{equation}
%\begin{equation}
%\label{eq:stereo_z2_projection}
%zope_{i} = \Vert  \begin{bmatrix}
%  \vec{n}_{i,l}^{(o)} \cdot (\vec{c}_{i,l}^{(o)} - \vec{c}_{i,r}^{(o)})  \\
%  \vec{n}_{i,r}^{(o)} \cdot (\vec{c}_{i,r}^{(o)} - \vec{c}_{i,l}^{(o)})
%\end{bmatrix}
%\Vert
%\end{equation}
and the \emph{up-vector projection error} $\delta_{y}$ according to equation \eqref{eq:stereo_y_projection}
\begin{equation}
\label{eq:stereo_y_projection}
\delta_{\vec{u},i} = \sqrt{\left( \vec{u}_{i,l}^{(o)} \cdot (\vec{c}_{i,l}^{(o)} - \vec{c}_{i,r}^{(o))}\right)^{2} + \left(\vec{u}_{i,r}^{(o)} \cdot (\vec{c}_{i,r}^{(o)} - \vec{c}_{i,l}^{(o))}\right)^{2}}.
\end{equation}
%\begin{equation}
%\label{eq:stereo_y2_projection}
%yope_{i} = \Vert  \begin{bmatrix}
%\vec{u}_{i,l}^{(o)} \cdot (\vec{c}_{i,l}^{(o)} - \vec{c}_{i,r}^{(o)})  \\
%\vec{u}_{i,r}^{(o)} \cdot (\vec{c}_{i,r}^{(o)} - \vec{c}_{i,l}^{(o)})
%\end{bmatrix}
%\Vert
%\end{equation}
The values $\delta_{\vec{u},i}$ and $\delta_{\vec{n},i}$ describe the relative registration error of the left and right camera w.r.t. to the viewing direction and the up-vector of the image plane. Due to the scale ambiguity of the baseline $b$, it is not possible to define a \emph{baseline projection error}. $\delta_{\vec{n},i}$ and $\delta_{\vec{u},i}$ reflect translation and orientation errors of the registered cameras. \\
We rank all registered stereo camera pairs according to the \emph{projection error } $\delta$ described in equation \eqref{eq:stereo_object_projection_error}
% \eqref{eq:stereo_z_projection} and \eqref{eq:stereo_y_projection} 
\begin{equation}
\label{eq:stereo_object_projection_error}
\delta_{i} = \sqrt{\delta_{\vec{n},i}^{2} + \delta_{\vec{u},i}^{2}}.
\end{equation}
We compute the scale ratios of the five lowest ranked stereo camera pairs (low rank means low $\delta_i$) according to equation \eqref{eq:stereo_scale_ratio_computation} and take the median of the scale ratios to deal with poorly stereo camera pairs, which coincidentally show a low $\delta$. Substituting $r$ in equation \eqref{eq:camera_to_object_point} allows us to compute an object motion trajectory consistent to the background reconstruction. \\


